Adversarial Predictions of Data Distributions Across Federated Internet-of-Things Devices

Federated learning (FL) is increasingly becoming the default approach for training machine learning models across decentralized Internet-of-Things (IoT) devices. A key advantage of FL is that no raw data are communicated across the network, providing an immediate layer of privacy. Despite this, recent works have demonstrated that data reconstruction can be done with the locally trained model updates which are communicated across the network. However, many of these works have limitations with regard to how the gradients are computed in backpropagation. In this work, we demonstrate that the model weights shared in FL can expose revealing information about the local data distributions of IoT devices. This leakage could expose sensitive information to malicious actors in a distributed system. We further discuss results which show that injecting noise into model weights is ineffective at preventing data leakage without seriously harming the global model accuracy.

==> pseudocode/fedavg.tex <==
\begin{algorithm}
\label{FedAvg}
\DontPrintSemicolon
\caption{Vanilla FedAvg~\cite{mcmahan2017communication}}

\SetKwFunction{FedAvg}{FedAvg}
\SetKwFunction{ClientUpdate}{ClientUpdate}
\SetKwProg{Fn}{Function}{:}{}


    initialize random global model weights, $w_0$\;
    \ForEach{round $t = 0, 1, 2, \cdots$}{
        $m \gets \max(C \cdot K, 1)$\;
        $S_t \gets \text{random subset of $m$ clients}$\;
        \ForEach{client $k \in S_t$ \textbf{in parallel}}{
            $w_{t + 1}^k \gets \mathit{ClientUpdate}(k, w_t)$\;
        }
        $m_t \gets \sum_{k \in S_t}n_k$\;
        $w_{t + 1} \gets \sum_{k \in S_t}\frac{n_k}{m_t}w_{t + 1}^k$\;
    }

    
    \setcounter{AlgoLine}{0}
    \SetKwProg{myproc}{Procedure}{}{}
    \myproc{ClientUpdate$(k,w)$}{
    % \Fn{\ClientUpdate{$k, w$}}{
        $\mathcal{B} \gets \text{(split $\mathcal{P}_k$ into batches of size $B$)}$\;
        \ForEach{local epoch $e=1, \ldots, E$}{
            \ForEach{batch $b \in \mathcal{B}$}{
                $w \gets w - \eta\nabla\ell(w; b)$\;
            }
        }
        \Return $w$ to server\;
    }
    
\end{algorithm}

==> sections/2_related_work.tex <==
\nathaniel{The related work section reads as a general related work section for FL in general. It does not feel focused on the problem of privacy of FL systems where the gradients/weights are intercepted by some adversarial entity. Maybe refining this section with this emphasis instead would be more impactful and relevant? I think the high-level overview of FL and FedAvg can be condensed and moved into the Introduction.}

The standard algorithm for federated learning, FedAvg, was proposed in ~\cite{mcmahan2017communication}. Later work~\cite{zhao2018federated, hsu2019measuring} noted that FedAvg tends to struggle with heterogeneous client data distributions, and several works since have explored modifications to the local update rule in FedAvg to mitigate these issues. For example, FedProx~\cite{li2020federated} adds a proximal term to the loss function to prevent local updates from drifting too far the global model, and SCAFFOLD~\cite{karimireddy2020scaffold} keeps track of server and client control variates to align client updates with the estimated direction of the global update. Rather than modifying the local update rule, some recent work has also shown that it is possible to improve upon FedAvg by modifying the client selection and aggregation steps: Wang et al.~\cite{wang2020optimizing} use reinforcement learning for client selection, selecting clients using a deep Q-network, and Xia et al.~\cite{xia2021auto} compute aggregation weights by using SGD. 

Recent research~\cite{zhu2019deep, zhao2020idlg, geiping2020inverting} has also indicated that sharing client gradient updates does not necessarily guarantee the privacy of client data. In particular, if a malicious actor sends a dummy input and label to a client's network, they can update the dummy input and label in a direction that increases the similarity between the gradient of the dummy input and label and the gradient sent by the client. This strategy has been shown to work even when the gradients come from a small batch of inputs. In the work reported here, instead of reconstructing client input samples, we demonstrate a method that can reconstruct client label distributions. Predicting a client's data distribution also has implications for strategies which attempt to reconstruct client images, because knowing the relative abundance of labels on a client allows for more intelligent predictions of the dummy label, and thus leads to a higher likelihood of success in reconstructing the images.

Another line of work studies federated learning settings in which the goal is to learn not only a global model, but also a personalized model for each client. Ditto~\cite{li2021ditto} learns both a global model and a local model for each client, while Stochastic Clustered Federated Learning~\cite{zeng2023stochastic} learns both a global model and personalized models for clusters of clients. Another work~\cite{collins2021exploiting} uses data from all clients to learn representations of input samples, while learning personalized heads for each client. Finally, Per-SSFL\cite{he2021ssfl} balances personalization and consensus among client models in a self-supervised setting. Because of the increasing popularity of unsupervised and self-supervised tasks, it is important to consider what (if any) privacy leakage might occur when client models are trained without labels. In this work, we focus on the case where the goal is to learn only a general global model, rather than models specific to each client.


%%%%%%%%%%%%%%%%%%%% 


